On the Abuse and Detection of Polyglot Files

A polyglot is a file that is valid in two or more formats. Polyglot files pose a problem for malware detection systems that route files to format-specific detectors/signatures, as well as file upload and sanitization tools. In this work we found that existing file-format and embedded-file detection tools, even those developed specifically for polyglot files, fail to reliably detect polyglot files used in the wild, leaving organizations vulnerable to attack. To address this issue, we studied the use of polyglot files by malicious actors in the wild, finding $30$ polyglot samples and $15$ attack chains that leveraged polyglot files. In this report, we highlight two well-known APTs whose cyber attack chains relied on polyglot files to bypass detection mechanisms. Using knowledge from our survey of polyglot usage in the wild -- the first of its kind -- we created a novel data set based on adversary techniques. We then trained a machine learning detection solution, PolyConv, using this data set. PolyConv achieves a precision-recall area-under-curve score of $0.999$ with an F1 score of $99.20$% for polyglot detection and $99.47$% for file-format identification, significantly outperforming all other tools tested. We developed a content disarmament and reconstruction tool, ImSan, that successfully sanitized $100$% of the tested image-based polyglots, which were the most common type found via the survey. Our work provides concrete tools and suggestions to enable defenders to better defend themselves against polyglot files, as well as directions for future work to create more robust file specifications and methods of disarmament.

==> background.tex <==
\section{Background}
file-formats
malware detection
static


background: why should you care?

The detection of malicious files can be hierarchically divided. At the highest level, methods are either static or dynamic. Static analysis treats a malicious file as a string of bytes, extracting features that consist of bytes of interest and byte metadata such as lengths, entropy, and Ngrams. Features for static analysis can be divided into format-agnostic and format-specific features. Format-agnostic methods focus on either the raw bytes of the file as it sits on-disk or on byte metadata that can be extracted from all files regardless of format, bearing in mind that all files are represented as a string of hexadecimal bytes. Format-specific features utilize the format specification for a given file type to extract only bytes which are significant to the structure or execution of that file type. For a Windows PE file, this would include imported functions from the import address table, section table entries, and a wide variety of fields from the \textit{COFF} and \textit{optional} headers. Static analysis is vulnerable to static obfuscation methods including but not limited to swapping equivalent opcodes, overwriting padding bytes, appending benign data, and altering optional fields in the file header NEED CITATIONS ARL papers.  Format-specific features are, potentially, less vulnerable to obfuscation as they correspond to structures necessary for the successful execution of the file. This provides more constraint on valid values, whereas format-agnostic features like length, entropy, and strings can be altered without damaging the functionality of the file.  

Dynamic analysis treats a malicious file as a set of observed behaviors. The file in question is executed in an isolated virtual machine (VM) known as a sandbox. As the file executes, metrics are collected such as changes to the file system, new processes, and registry key alterations. Dynamic analysis, with two significant exceptions, is not vulnerable to static obfuscation methods since it ignores a file sample's on-disk representation. However, dynamic analysis can be evaded using sandbox evasion techniques. This family of methods delays or cancels execution of the malware. Delay-based methods exploit the time constraint imposed on any malware detector by modern enterprises. The malware simply delays execution in the hopes that the dynamic detector will halt the examination before any malicious activity is detected. Alternatively, the malware file may attempt to identify the running environment. Virtual machines can leave behind tell-tale signs such as a sparse file system, constrained storage/RAM, and unusual running processes. If these signs are detected by the malware, it may halt execution to avoid detection. Thus dynamic detection, while robust to static obfuscation, has its own set of vulnerabilities. 

The two exceptions mentioned previously are packing and polyglots. Packing refers to the process of compressing and/or encrypting a file's contents. Although this is a static alteration, the addition of decompression/decryption code to an existing file also alters the dynamic behavior of the file. In this manner, packing is an obfuscation method that affects both static and dynamic analysis. 

Polyglots are also a static alteration that can affect dynamic analysis in a unique way. A polyglot is a single file that is fully valid in two or more file formats. This means the polyglot is interpreted and executed differently depending on which program loads the file. The question of which format's contents will be executed automatically depends on the specific version of the operating system.  -NEED experiment to prove this. might add some punch to this paper, might be too time-consuming. talk to sean.




